ACP+: An Age Control Protocol for the Internet

We present ACP+, an age control protocol, which is a transport layer protocol that regulates the rate at which update packets from a source are sent over the Internet to a monitor. The source would like to keep the average age of sensed information at the monitor to a minimum, given the network conditions. Extensive experimentation helps us shed light on age control over the current Internet and its implications for sources sending updates over a shared wireless access to monitors in the cloud. We also show that many congestion control algorithms proposed over the years for the Transmission Control Protocol (TCP), including hybrid approaches that achieve higher throughputs at lower delays than traditional loss-based congestion control, are unsuitable for age control.

==> algorithm_draft.tex <==
\section{The ACP+ Control Algorithm}
\label{sec:algorithm}

Let the control epochs of ACP+ be indexed $1,2,\ldots$. Epoch $k$ starts at time $t_k$ and ends at $t_{k+1}$, which is the beginning of the next epoch. Let $\lambda_k$ be the update rate set by the control algorithm for epoch $k$. The source ACP transmits updates at a fixed time period of $1/\lambda_{k}$ seconds in the interval $(t_{k}, t_{k+1})$. For the first control epoch, beginning at $t_1$, the update rate $\lambda_{1}$ is set to the inverse of the average packet round-trip-times (RTT) obtained at the end of the initialization phase. %At time $t_k$, $k>1$, the update rate is set to $\lambda_k$. The source transmits updates at a fixed period of $1/\lambda_{k}$ in the interval $(t_{k}, t_{k+1})$.

The length $\mathcal{T}_k=t_{k+1}-t_k$ of the $k\textsuperscript{th}$ control epoch is set as an integral number $\eta$ of time periods, each of length $1/\lambda_k$. That is $\mathcal{T}_k= \eta/\lambda_k$. A control epoch should be long enough to allow for reasonable estimates of the time-average age and backlog that result from setting the update rate to $\lambda_k$ for epoch $k$. In this work, we find $\eta=10$ to work well for all our chosen scenarios in simulations and real-world experiments. %A larger $\eta$, for a given update rate $\lambda_k$, would result in longer control epochs and slower adaptation by the algorithm. A smaller $\eta$ results in shorter control epochs. However, a short control epoch may not be sufficient to estimate well the impact of the update rate $\lambda_k$ set for epoch $k$. In this work, we set $\eta=10$. %\edit{The next epoch starts at $t_{k+1}$. The length of the control epoch is set as $\mathcal{T}_k=t_{k+1}-t_k=\eta/\lambda_k$. In this work, we fixed the value of $\eta=10$ such that atleast 10 packets are sent by the source using updated $\lambda_{k}$.}\RY{I think we need to say explain how we decide $t_{k+1}$ starts. Later on, I know we explain that $\mathcal{T}=t_{k+1}-t_k=10/\lambda_k$. It seems like we should say that here. Although maybe we should have 10 be replaced by a parameter? It's not clear to me that 10 is a good number in all scenarios?}

Let $\overline{\age}_k$ be the estimate at the  ACP+ source at time $t_k$ of the time average update age at the monitor  over the interval $(t_{k-1}, t_k)$. To calculate it, the ACP+ source must construct its estimate of the age sample function (see Figure~\ref{fig:ageSampleFunction}), over the interval, at the monitor. It knows the time $a_i$ the source sent a certain update $i$. However, it needs the time $d_i$ at which update $i$ was received by the monitor, which it approximates by the time the ACK for packet $i$ was received. On receiving the ACK, it resets its estimate of age to the resulting round-trip-time (RTT) of packet $i$. The time average $\overline{\age}_k$ is obtained simply by calculating the area under the resulting age curve over $(t_{k-1}, t_k)$ and dividing it by $t_k - t_{k-1}$. 
%\del{Note that this value is an overestimate of the age of the update packet when it was received at the monitor, since it includes the time taken to send the ACK over the network.}
Resetting the estimate of age to the RTT overestimates the true age of the update packet, when it was received at the monitor, by the time taken to send the ACK from the monitor to the source. However, this estimate doesn't require any time synchronization between the ACP source and monitor. Further, the overestimation offsets the time-average age by the one-way delay, from the monitor to the source, suffered by the ACK, and doesn't affect the update rate that minimizes the average age. This has also been shown in~\cite{uysal_practice_2021}. %
%\edit{Additionally, this overestimate does not affect the optimal operating point as we consider a linear age sample function~\cite{uysal_practice_2021}.}
%\RY{We need a sentence explaining why an overestimate is OK.}

\begin{figure}[!t]             
	\begin{center}
		\includegraphics[width=0.45\textwidth]{Figs/Backlog.pdf}
		\caption{A sample function of the backlog process $B(t)$. Updates are indexed $1,2,\ldots$. The timestamp of update $i$ is $a_i$. The time at which update $i$ is received by the monitor is $d_i$. Since update $3$ is received before $2$, backlog is reduced by $2$ packets at $d_3$. Also, there is no change in $B(t)$ at $d_2 > d_3$.}
		\label{fig:backlogSampleFunction}
	\end{center}
\end{figure}

% \begin{figure}[!t]             
% \begin{center}
% \includegraphics[width=0.5\textwidth]{Figs/flowchart_final.pdf}
% \caption{Update of $\overline{\RTT}$, $\overline{Z}$, $\overline{T}$, $\Delta(t)$, and $B(t)$, which takes place every time an ACK is received by the source ACP+. \RY{This is just a collection of equations that should be in the text, not in a figure.}}
% \label{fig:flow}
% \end{center}
% \end{figure}

Let $\overline{B}_k$ be the time average of backlog calculated over the interval $(t_{k-1}, t_k)$. This is the time average of the instantaneous backlog $B(t)$ over the interval. 
%Figure~\ref{fig:backlogSampleFunction} shows the sample function of the backlog process $B(t)$. 
The instantaneous backlog increases by $1$ when the source sends a new update. When an ACK corresponding to an update $i$ is received, update $i$ and any unacknowledged updates older than $i$ are assumed ACKed %($\text{ACKed}_{updates}$ in Figure~\ref{fig:flow}) 
and removed from the instantaneous backlog. Figure~\ref{fig:backlogSampleFunction} shows the instantaneous backlog corresponding to the age sample function in Figure~\ref{fig:ageSampleFunction}. 

% In addition to using RTT(s) of updates for age estimation, we also use them to maintain an exponentially weighted moving average (EWMA) $\overline{\RTT}$ of RTT. We update $\overline{\RTT} = (1 - \alpha) \overline{\RTT} + \alpha \RTT$ on reception of an ACK that corresponds to a round-trip-time of RTT. % uses an estimate of the average time between consecutive update arrivals at the monitor. Specifically, it 
% The source ACP+ also estimates the inter-update arrival times at the monitor and the corresponding EWMA $\overline{Z}$. The inter-update arrival times are approximated by the corresponding inter-ACK arrival times.
% The source updates $\overline{\RTT}$ and $\overline{Z}$ every time an ACK is received. 

\RY{I found this section pretty confusing/vague. I tried to write it more precisely in the following, but I'm kinda stuck. For example, if updates arrive out of order, I understand that missing updates are ACKED by a fresher update ACK, but how are missing inter-update times $Z$ computed? Here is my initial attempt to be more precise:}

Starting at time $t=0$, a sequence of fresh updates indexed $i=1,2,\ldots$ arrive at the source with the $i$th update arriving at time times $a_i$. When update $i$ is received at the monitor at time $d_i$, an  update ACK is transmitted back to the source, arriving at time $\dhat_i$  with corresponding RTT 
\begin{equation}
\RTT_{i}=\dhat_i-a_i.
\end{equation}
At the source, the received ACKs are used to construct approximations $\agehat(t)$ and $\Bhat(t)$ of the age process $\age(t)$ and the backlog process $B(t)$. To estimate $B(t)$, we define 
\begin{subequations}
\begin{align}
S(t)&=\max\set{i\colon a_i\le t},\\
\Nhat(t)&=\max\{i\colon \dhat_i\le t\}. 
\end{align}
\end{subequations}
At time $t$, $S(t)$ is the index of the freshest update that has been transmitted and $\Nhat(t)$
is the index of the freshest update that has been ACKed at the source. We say an  ACK $i$ arriving at time $t=\dhat_i$ is {\em fresh} if it advances the ACK counter $\Nhat(t)$. The estimated backlog at time $t$ is
\begin{equation}
    \Bhat(t)=S(t)-\Nhat(t).\eqnlabel{estimatedB}
\end{equation}
In \eqnref{estimatedB}, the estimated backlog increases by $1$ when the source sends a new update at time $t=a_i$. Furthermore, only fresh ACKs reduce the estimated backlog. In particular, when the source receives a fresh ACK corresponding to an update $i$, update $i$ as well as any unacknowledged updates older than $i$ are ACKed 
%($\text{ACKed}_{updates}$ in Figure~\ref{fig:flow}) 
and removed from the estimated backlog. This estimated backlog is a conservative estimate in that updates are removed from the backlog only when updates ACKs are returned to the source. To estimate the age process at the source, we define
\begin{equation}\eqnlabel{agehat}
    \agehat(t)=t- a_{\Nhat(t)}.
\end{equation}
The effect of \eqnref{agehat} is that only fresh ACKs reduce the estimated age $\agehat(t)$. Moreover, if ACK $i$ arriving at time $t=\dhat_i$ is fresh, then $\agehat(\dhat_i)=\RTT_i$.

In addition to using update ACKs for age and backlog estimation, we also use them to maintain  exponentially weighted moving averages (EWMAs) $\overline{\RTT}$ and $\overline{Z}$ of the RTT and the ACK interarrival time.  
%Our approach is to approximate the inter-update arrival times $d_{i}-d_{i-1}$ (at the monitor)  by the corresponding inter-ACK  times $Z_{i}=\dhat_{i}-\dhat_{i-1}$ at the source.
On receipt of an ACK of update $i$ at time $t=\dhat_i$, the ACK inter-arrival time is estimated as
\begin{equation}
 Z_i=\dhat_i-\dhat_{\Nhat(t)}\ \text{\RY{This guess works ok if ACKs arrive in order}}
\end{equation}
The source updates $\overline{\RTT}$ and $\overline{Z}$ every time an ACK is received, specifically,
\begin{subequations}
\begin{align}
    \overline{\RTT}(t) &= (1 - \alpha) \overline{\RTT}(t^-) + \alpha \RTT_i,\\
    \overline{Z}(t) &=(1-\alpha)\overline{Z}(t^-)+\alpha Z_i,
\end{align}
\end{subequations}
In the absence of an ACK, $\overline{\RTT}(t)$ and $\overline{Z}(t)$ remain unchanged.

%The length of a control epoch is set as $\mathcal{T} = 10/\lambda_{k}$. Thus at least $10$ packets are sent by the source using the updated $\lambda_{k}$. 

\RY{Does the epoch end when the 10th update is sent?} 
\edit{I vaguely get the statement below. In my understanding we replace $\mathcal{T}$ by $\mathcal{T}_k$. Confirm this!}
\RY{Since $\lambda_k$ keeps changing, $\mathcal{T}$ keeps changing. My suggestion is we define $\mathcal{T}_k$ as the interval $(t_{k-1},t_k)$ and $\tau_k=t_k-t_{k-1}$ as the length of the $k$th interval.}
%\edit{We define $\mathcal{T}_k$ as the length of the control epoch $(t_{k-1},t_k)$ and $\tau_k=t_k-t_{k-1}$ as the length of the $k$th epoch.}
At time $t_k$, the source ACP+ calculates the difference $\delta_k = \overline{\age}_k - \overline{\age}_{k-1}$ in average age measured over epochs $(t_{k-1}, t_k)$ and $(t_{k-1}, t_{k-2})$. Similarly, it calculates $b_k = \overline{B}_k - \overline{B}_{k-1}$.
ACP+ at the source chooses an action $u_k$ at the \edit{beginning of} $k$\textsuperscript{th} epoch that targets a change $b^{*}_{k+1}$ in average backlog over an interval of length $\mathcal{T}_k$ with respect to the $k$\textsuperscript{th} \del{interval} \edit{epoch}.

\RY{The $k$th epoch is the same thing as the $k$th interval?? I think we should try to use one term or the other but not both.}
The actions, may be broadly classified into additive increase (INC), additive decrease (DEC), and multiplicative decrease (MDEC). MDEC corresponds to a set of actions $\set{\text{MDEC}(\gamma)\colon \gamma=1,2,\ldots}$. Specifically,
\begin{subequations}
\begin{align}
\text{INC}\colon&  b^{*}_{k+1} = 1,\\
\text{DEC}\colon&  b^{*}_{k+1} = -1,\\
\text{MDEC}(\gamma)\colon&  b^{*}_{k+1} = -(1 - 2^{-\gamma}) B_k.
\end{align}
\end{subequations}

\begin{algorithm}[t]
\caption{ACP+ Control Algorithm}
\label{alg:acp+}
%\footnotesize
%\RY{Maybe the pseudo-code should identify $b_k$ and $\delta_k$ as the input?}
\begin{algorithmic}[1]
\State \textbf{INPUT:} $b_k$, $\delta_k$ 
\State \textbf{INIT:} $\text{flag} \gets 0$, $\gamma \gets 0$
\While{true} 
	\If {$b_k>0$  \&\& $\delta_k >0$}\label{alg:one}
		 \If {$\text{flag}==1$}
		 \State $\gamma=\gamma+1$\label{alg:oneincr}
			\State MDEC($\gamma$): $b^{*}_{k+1} = -(1 - 2^{-\gamma}) B_k$
		\Else
			\State DEC: $b^{*}_{k+1} = -1$ \label{alg:oneDEC}
		\EndIf
		\State $\text{flag}\gets 1$
	\ElsIf { $b_k>0$  \&\& $\delta_k <0$}\label{alg:two}
	        \State INC: $b^{*}_{k+1} = 1$
			\State $\text{flag}\gets 0$,
			$\gamma\gets0$ \label{alg:two2}
	\ElsIf { $b_k<0$  \&\& $\delta_k >0$}\label{alg:three}
	    \State INC: $b^{*}_{k+1} = 1$
		\State $\text{flag}\gets 0$, $\gamma\gets0$ 
	\ElsIf { $b_k<0$  \&\& $\delta_k <0$}\label{alg:four}
		 \If {$\text{flag}==1$ \&\& $\gamma>0$}
			\State MDEC($\gamma$): $b^{*}_{k+1} = -(1 - 2^{-\gamma}) B_k$ \label{alg:fourMDEC}
		\Else
		    \State DEC: $b^{*}_{k+1} = -1$
			\State $\text{flag}\gets 0$, $\gamma\gets0$
		\EndIf
	\EndIf
% \State update $\lambda_k$
\State \Call{UpdateLambda}{$b^{*}_{k+1}$} \label{alg:update}
\State wait $\overline{T}$ 	
\EndWhile
\Statex
\Function{UpdateLambda}{$b^{*}_{k+1}$}
% \State \textbf{INIT:} 
% $\overline{\RTT} = (1 - \alpha) \overline{\RTT} + \alpha \RTT$,
% $\overline{\text{Z}} = (1 - \alpha) \overline{\text{Z}} + \alpha \text{Z}$
\State $\lambda_k = \frac{1}{\overline{Z}} + \frac{b^{*}_{k+1}}{\mathcal{\overline{\RTT}}}$ \label{alg:calc}
% \State
% $\lambda_k = \max( 0.75 * \lambda_{k-1}, \min(\lambda_{calc}, 1.25 * \lambda_{k-1}))$
	\If {$\lambda_k < 0.75*\lambda_{k-1} $}\label{alg:min}
		 \State 
		 $\lambda_k = 0.75*\lambda_{k-1}$
		 \Comment{Minimum $\lambda$ threshold}
	\ElsIf {$\lambda_k > 1.25*\lambda_{k-1} $}\label{alg:max}
	        \State
	        $\lambda_k = 1.25*\lambda_{k-1} $
			\Comment{Maximum $\lambda$ threshold}
% 	\Else
% 	      \State
% 		  $\lambda_k = \lambda_{calc} $ 
	\EndIf
\State
\Return $\lambda_k$
\EndFunction
\end{algorithmic}
\end{algorithm}

ACP+ attempts to achieve $b^{*}_{k+1}$ by setting $\lambda_k$ appropriately. The estimate of $\overline{Z}$ at the source ACP+ of the average inter-update arrival time at the monitor gives us the rate $1/\overline{Z}$ at which updates sent by the source arrive at the monitor. This and $\lambda_k$ allow us to estimate the average change in backlog over $\mathcal{T}_k$ as $(\lambda_k - (1/\overline{Z})) \mathcal{\overline{\RTT}}$. \RY{It seems to me this is the average change in the backlog over one RTT rather than $\mathcal{T}_k$?} \SKK{May be we should just say the desired change in average backlog is $(\lambda_k - (1/\overline{Z})) \mathcal{\overline{\RTT}}$.}
\RY{Our protocol is epoch-based and our words say we are targeting a certain change in backlog over an epoch. What happens if we replace $\overline{RTT} with $$\mathcal{T}$ in eqn (8). Does it make a difference? I'm not proposing a total do-over. I'm just trying to understand. }\SKK{We are interested in changing the time-average backlog. The desired change $b^{*}_{k+1}$ is in fact the desired change in the time-average backlog. The equation above is based on the fact that the time-average backlog is the product of the time-average system time and the arrival rate. So the term should be $\mathcal{\overline{\RTT}}$. We are assuming that time-averages realize themselves well enough over $\mathcal{T}$. Hope this makes things a tad more clear.}
Therefore, a desired change of $b^{*}_{k+1}$ requires choosing %$\lambda_k = \frac{1}{\overline{Z}} + \frac{b^{*}_{k+1}}{\mathcal{\overline{\RTT}}}$. 
\begin{align}
\lambda_k = \frac{1}{\overline{Z}} + \frac{b^{*}_{k+1}}{\mathcal{\overline{\RTT}}}.
\end{align}



Algorithm~\ref{alg:acp+} summarizes how ACP+ chooses its action $u_k$ as a function of $b_k$ and $\delta_k$. The source ACP+ targets a reduction in average backlog over the \edit{length next control epoch} \del{interval} in case either $b_k,\delta_k>0$, 
%$\delta_k>0$ 
or $b_k,\delta_k<0$
%\delta_k<0$. 
Both $b_k$ and $\delta_k$  positive, (line~\ref{alg:one} in Algorithm~1) indicates that the update rate is such that updates are experiencing larger than optimal delays. In this case, ACP+ attempts to reduce the backlog, first using DEC (line~\ref{alg:oneDEC}), followed by multiplicative reduction MDEC to reduce congestion delays, and in the process reduce age quickly. Consecutive occurrences ($\text{flag} == 1$) of this case (tracked by increasing $\gamma$ by $1$ in line~\ref{alg:oneincr}) attempt to decrease backlog even more aggressively, by a larger power of $2$.


The condition that $b_k$ and $\delta_k$ are both negative (line~\ref{alg:four}) corresponds to a reduction in both age and backlog. ACP+ greedily aims at reducing backlog further in the hope that age will reduce too. It attempts MDEC (line~\ref{alg:fourMDEC}) if previously the condition $b_k,\delta_k>0$ was satisfied; otherwise, it attempts the additive decrease DEC.

The source ACP+ targets an increase in average backlog over the next control \del{interval} \edit{epoch} in case either $b_k>0, \delta_k<0$ or $b_k<0, \delta_k>0$. On the occurrence of the first condition (line~\ref{alg:three}) ACP+ greedily attempts to increase backlog. The condition $b_k<0, \delta_k>0$ hints at too low an update rate causing an increase in age. So, ACP+ attempts an additive increase (line~\ref{alg:two2}) of backlog.
%Figure~\ref{fig:acpDemo} shows a snippet of ACP in action.

% \begin{figure}[!t]             
% 	\begin{center}
% 		\includegraphics[width=0.4\textwidth]{Figs_acpv1/ACPDemo2}
% 		\caption {A snippet from the functioning of ACP+. \edit{We can remove this, it is not communicating anything apart from that it works.}%The y-axis of the plot showing actions denotes the action and the line number in Algorithm~\ref{alg:acp+}. %Note the action marked by the dotted red line. At the time instant ACP observes an increase in both backlog and age and chooses ($9$,DEC) initially. However, there is still a significant jump in age. This results in the choice of multiplicative decrease ($7$,MDEC).
% 		}
% 		\label{fig:acpDemo}
% 	\end{center}
% %	\vspace{-0.2in}
% \end{figure}


==> background_tcp.tex <==
\section{Primer on TCP Congestion Control}\label{sec:congestion}
%\textbf{Primer on TCP Congestion Control.}
Congestion control was introduced in the Internet in 1980s to overcome the congestion collapse of the Internet~\cite{rfc793}. These algorithms help achieve higher utilization of the available network bandwidth while avoiding overloading the network. Over the years, the design strategies of the congestion control have evolved from loss-based to delay-based and now recently introduced hybrid strategies to improve the TCP's performance in different networks such as lossy wireless or in the presence of large network buffers. 
%trying to improve the performance for a specific network. 

The \textbf{loss-based}  strategies aim for high throughput by having as many packets as possible in each queue without exceeding the available queue occupancy. This allows an end-to-end flow to achieve a rate equal to the bottleneck bandwidth; however, this is at the expense of large delays and eventual losses due to excessive queueing at the bottleneck.
These algorithms generally have a slow start phase followed by a congestion avoidance phase. 
A few examples of loss-based congestion control algorithms are Reno, NewReno~\cite{rfc5681}, Highspeed-TCP~\cite{rfc3649}, Scalable TCP \cite{scalabletcp2003}, TCP Westwood~\cite{mascolo2001tcp}, TCP Westwood$+$~\cite{MASCOLO200493}, BIC~\cite{xu2004binary} and CUBIC~\cite{ha2008cubic}. CUBIC is the current default congestion control algorithm in the Linux kernel. CUBIC differs from the traditional congestion control algorithms like Reno/NewReno in setting the congestion window size as a cubic function. It employs a fast recovery after the loss event and is less aggressive as it approaches the \texttt{cwnd\_max}, making it suitable for flows that require higher bandwidth. CUBIC offers high RTT-fairness where RTT fairness is a fairness measure among connections with different RTTs sharing the link. This is because the \texttt{cwnd} calculation is independent of RTT. However, it fails to achieve maximum available bandwidth utilization and leads to packet losses due to it's congestion detection mechanism.

The \textbf{delay-based} strategies monitor the delay over the Internet using the RTT measurements and aim to keep the queueing delays below a certain threshold and avoiding the large delays associated with the loss-based approaches. These are proactive schemes instead of the reactive loss-based approaches. The use of delay (instead of losses) as a congestion indicator helps avoid queue buildup which in turn are advantageous for low-latency applications. Additionally, these mechanisms avoid the throughput oscillations associated with the Additive Increase Multiplicative Decrease (AIMD) based approaches such as CUBIC. However, RTTs based congestion approaches suffer due to delayed ACKs, cross traffic and queues in the network.
A few examples of these are Vegas~\cite{brakmo1994tcp}, FAST~\cite{jin2005fast}, TCP LoLa~\cite{hock2017tcp} and TIMELY~\cite{mittal2015timely}. 
%Since Vegas is the basic delay based algorithm, we will describe it in some detail in this text.
Vegas uses RTT measurements to estimate the buffer occupancy at the bottleneck queue as a function of expected and actual transmission rate, and attempts to keep it under a predefined threshold~\cite{h2h_compSurvey2010}. $RTT_{\text{base}}$ is used as a baseline measurement for a congestion-free network. The theoretical maximum expected transmission rate in a congestion free network is \texttt{cwnd/$RTT_{\text{base}}$}. A Vegas flow will achieve this rate if all transmitted packets are acknowledged within the minimum RTT such that $RTT_{\text{i}}$=$RTT_{\text{base}}$, where $RTT_{\text{i}}$ is the RTT of $i^{th}$ packet. Similarly, the actual transmitted rate is calculated using the currently measured RTT as \texttt{cwnd/$RTT_{\text{i}}$}. Therefore the number of packets queued at the bottleneck can be calculated as
\[
    \Delta = \texttt{cwnd}\frac{RTT_{\text{i}}-RTT_{\text{base}}}{RTT_{\text{i}}}
\]

At reception of each ACK, Vegas calculates $\Delta$ and keeps it between predefined thresholds $\alpha$ and $\beta$. For Linux kernel, $\Delta$ values lies between $2-4$. A $\Delta$ value higher than $\beta$ indicates congestion and the \texttt{cwnd} is reduced by one. If $\Delta$ is lower than $\alpha$, \texttt{cwnd} is increased by one.  

Vegas minimizes the queueing delays and reduce throughput oscillations, resulting in improvements in long term throughput averages. Despite having these benefits, Vegas suffers from some inherent issues. First, the algorithm has a slow growth rate and therefore can lead to under-utilization of resources in a high speed network. Secondly, the algorithm uses RTT measurements to calculate the sending rate and any change in the network leading to an increase in RTT is interpreted as congestion and results in a unnecessary reduction in the sending rate.
Finally, it doesn't work well when other loss-based flows are sharing the network and switches to a loss-based approach in this scenario.
%A new class of hybrid congestion control algorithms emerged from the low latency requirements.

\textbf{Hybrid} algorithms use the combination of loss and delay as congestion indicators.
While the loss-based strategies work well in a high speed network with low resource utilizations as these can quickly ramp up the the \texttt{cwnd} sizes, the delay-based schemes are more suited for a higher utilization congested networks. The basic idea behind the hybrid approach was to improve on the loss-based strategies such that congestion is detected much before the queues build up and the packets are dropped yet keeping the throughput and network utilization high. A few examples include TCP Compound~\cite{tan2006compound}, Veno~\cite{fu2003tcp}, Illinois~\cite{liu2008tcp} and YeAH~\cite{baiocchi2007yeah}. 

In 2016, Google proposed the \textbf{bottleneck bandwidth and round-trip time (BBR)}~\cite{cardwell-bbr-2016} congestion control algorithm which aims to utilize available network bandwidth without filling network pipes. BBR periodically estimates available network bandwidth ($BW_{\text{Btl}}$) using the maximum data delivery rate and baseline round-trip time ($RTT_{\text{base}}$). As shown in Figure~\ref{fig:TCPtransient_SteadyState}, in a deterministic network environment, working at this point can ensure maximum data delivery rate with minimum congestion.
BBR uses four different phases for its operation, namely \texttt{startup}, \texttt{drain}, \texttt{probe bandwidth} and \texttt{probe RTT}. The \texttt{startup} phase uses the slow start mechanisms of loss-based algorithms, essentially doubling the sending rate every RTT. BBR uses the received ACKs to estimate the current delivery rate. BBR assumes that the bottleneck rate is achieved when the delivery rate stops increasing for \textit{three} consecutive RTTs. This marks the end of \texttt{startup} phase and BBR enters the \texttt{drain} phase to remove excess queue buildup in the previous sending cycle. BBR reduces its sending rate to $0.75\times BW_{\text{Btl}}\times RTT_{\text{base}}$. BBR calculates the RTT of the every received ACK and sets $RTT_{\text{base}}$ as the minimum value of RTT in the past 10 seconds. The \texttt{cwnd} is set to the bandwidth delay product (BDP).
\[
    \texttt{cwnd}= BW_{\text{Btl}}\times RTT_{\text{base}}.
\]
To adapt to the changing network conditions, BBR periodically launches the \texttt{probe bandwidth} phase by sending data at a higher rate ($1.25\times BDP$) for an RTT interval. This is followed by a new \texttt{drain} phase where rate is reduced to drain the excess queues formed. This is done once every eight cycles each lasting for $RTT_{\text{base}}$ duration. If the $RTT_{\text{base}}$ is same for past 10 seconds, BBR enters the \texttt{probe RTT} phase and reduces the in-flight data to four packets in order to drain the bottleneck queue entirely. This phase lasts for 200 ms. BBR is designed to spend majority of time in \texttt{probe bandwidth} with \texttt{probe RTT} being triggered for $\approx 200ms$ once every 10 seconds. 

==> fairness.tex <==
% \subsection{Age Fairness Using ACP+}
% \label{sec:fairness}
% % Lastly, we observe that ACP+ is \textit{age fair} with Jain's fairness index \cite{jain1984quantitative} reducing from about $.99$ to $.89$ as we increase source density from $6$ to $48$ nodes.
% We quantify fairness in age achieved by multiple ACP+ sources that share an access network and send their updates to a monitor. %Fairness is critical to determine if all the ACP flows are getting a fair share of the end-to-end network path. The primary purpose of our fairness analysis is to check the compatibility of the ACP+ with other existing ACP+ sources in the network, which are unknown to ACP+. 
% We use the Jain's fairness index~\cite{jain1984quantitative} to quantify \textit{age fairness} in both our simulations and real-world experiments. The Jain's fairness index can take values between $0$ and $1$. A larger fairness index implies more similar ages of the different sources at the monitor. An index of $1.0$ indicates that the ACP+ control algorithm enables the ACP+ flows to achieve the same ages over their paths to the monitor.

% In our simulations, we find that as we increase the number of sources sharing the network from $6$ to $48$, our fairness index reduces from $.99$ to $.89$. In our real-world experiments, the fairness index lies between $.99$ to $1.0$ as we increase source density from $2$ to $80$ for all the WiFi link rates ($6$, $12$ and $24$ Mbps). ACP+ ensures age fairness in our experiments.
